Too Noisy To Learn: Enhancing Data Quality for Code Review Comment Generation

Code review is an important practice in software development, yet it is time-consuming and requires substantial effort. While open-source datasets have been used to train neural models for automating code review tasks, including review comment generation, these datasets contain a significant amount of noisy comments (e.g., vague or non-actionable feedback) that persist despite cleaning methods using heuristics and machine learning approaches. Such remaining noise may lead models to generate low-quality review comments, yet removing them requires a complex semantic understanding of both code changes and natural language comments. In this paper, we investigate the impact of such noise on review comment generation and propose a novel approach using large language models (LLMs) to further clean these datasets. Based on an empirical study on a large-scale code review dataset, our LLM-based approach achieves 66-85% precision in detecting valid comments. Using the predicted valid comments to fine-tune the state-of-the-art code review models (cleaned models) can generate review comments that are 13.0% - 12.4% more similar to valid human-written comments than the original models. We also find that the cleaned models can generate more informative and relevant comments than the original models. Our findings underscore the critical impact of dataset quality on the performance of review comment generation. We advocate for further research into cleaning training data to enhance the practical utility and quality of automated code review.

==> arxived_draft.tex <==
\section{INTRODUCTION} 

% focusing on the practical side 

% key message: 

% 1. P1: 
%     1. what’s the goal of code summarization, who can benefit from code summarization;
%     2. the necessity of large-scale and high-quality datasets for learning based models 
%     3. Many datasets mined from real-world project repositories (GitHub) has been constructed. Models are trained and evaluated on them. 
% 2. P2: 
%     1. the datasets contain noise, from **differences in coding conventions and assumptions employed in modern programming languages and IDEs, as well as ad hoc nature of development processes and practices [54]**
%     2. e.g., multi-lingual natural languages → increasing the complexity of understanding the code 
%     3. existing studies confirmed some types of noise: such as auto-generated code [30], TODO comments [14], and incomplete comments [60]. 
%     4. Particularly, Steidl et al 
% 3. Motivation: to investigate the concern of data quality for code summarization
%     1. systematic study to **assess and improve the quality of four datasets** 
%     2. research methodology overview: four steps  
%         1. a taxonomy of 12 noisy types 
%         2. rule-based cleaning tool 
%         3. asses the dataset quality 
%         4. impact of noises on three code summarization models 
%         5.



% 
% In the first paragraph, we introduce what's the goal of code review, who benefit from code review. 
% The intention of code review has 
% can we add some examples to make it concrete 

%P1: introduce the significance of automate code review and the source of construcing datasets 
xx has shown that code review is useful for practitioners to identify the deep logic bugs, improve software quality and beneficial for knowledge transfer. 
At the core part of the code review, reviewer's feedback as expressed in natural language serve as the bridge to realise this. However, this process is often time-consuming and takes a lot of effort. xx has reported that developers spend xx of their time for code review. 
To reduce the burden of human reviewers, recent work in has been focusing on automating code review comment generation by training neural models on large-scale datasets. 
These datasets are often constructed from real-life projects in open-source platforms such as GitHub. 
For example, Li et al., (2022) mined xxK datasets over xx projects and Tufano et al., (2021) mined xx instances from Gerrit. Many follow-up models has been trained and evaluated based on these datasets. 

%P2: Introduce the problem of dataset quality: noise exist in datasets and what's the consequence or concern
% TODO: need defintion for noisy 

Although much effort has been put into cleaning the datasets, such as removing bots, filtering out noisy comments using heuristics, xx and xx. 
However, recent work (Tufano et al., 2024) raised concerns about the quality of three popularly used datasets and pointed out that the noise persistent in these datasets. 
This is not ideal. As these datasets are used to train and evaluate models. 
Correspondingly, models trained on noisy data will capture the noise inside the data, and generate comments that are less practically useful when being used in real-life by practitioners. 
On the other hand, existing works rely on human review comments as ground truth to evaluate the performance of code review comment generation models, while the existence of noisy comments means that the evaluation will not reflect the true needs of practitioners. 

%P3: point out the challenge of identifying noisy comments. 
Although many has been shown that the high-quality dataset has big impact on training high-performing neural models in various context [xx]. Identifying the noise code review comments remains to be a challenge as it requires deep understanding of both the code changes, natural language comments and the interaction between them. Understanding the code changes involve prior knowledge in both code and potentially project specific knowledge, while understanding the semantics in review comments is also a challenge as it could be ambiguous, requiring inference. 

Inspiring by the recent advancements in large-language models that are pre-trained on multiple sources datasets such as text-corpora and code, they has shown promising performance on understanding the both code and language on various benchmarks []. Many recent work has been shown that LLMs can be used for data annotation. 
In this paper, we propose to leverage the power of large-language models to clean noisy data and then assess the impact of noisy data on comment generation models. 


% However, recent work (Tufano et al., 2024) pointed out that these datasets are noisy due to various reasons, such as
% not asking for code changes, 


% concerns: 
% existing works using human comments as ground truth to evaluate model performance 
% however, as xx pointed out, the quality of code review comments vary, many noisy comments exist. 
% This raises concerns regarding in evaluation, because we don't know what we really want our model to generate. 

% On the other hand, 

% Code review comments are important for practitioners. If our trained model only generate meaningless or unreliable comments, which will not be 

% On the other side, the quality of code review comments is also important for training models to 
% In this study, we 
% Due to this, the performance of classification may degrade [14].


% \section{Approach}

Our main contributions are: 
\begin{itemize}
    \item We found the 36\% comments in the code reviewer dataset are noisy and show that 11.5\% - 21.4\% noisy in code review comments can be effectively removed by leveraging the recent large-language models. Our cleaned dataset will be publicised for future research. 
    \item We empirically show that by removing noisy comments can improve models' performance on code review comment generation models. {\color{blue} emphasise the codeT5 vs CodeReviewer.}. 
    \item Our deep analysis on the generated comments on original and cleaned datasets show that xx types of comments benefited most, highlighting the importance of high-qualiy dataset.
\end{itemize}

\textbf{Open Science} To support future work on , the replication package, including the data we cleaned using large langauge models, the experimental results and scripts are available at [TODO].


\textbf{Open Science:} To facilitate reproducibility and foster further research, we provide the replication package at [TODO]. This package includes cleaned datasets, experimental results, and scripts, enabling researchers to build upon our work in advancing automated code review.

\textbf{Paper Organization:} The remainder of this paper is structured as follows: Section~\ref{sec:study_design} outlines the overview of our study design. In Section~\ref{sec:identifying_noisy_comments_rq1} presents our approach to identifying noisy comments in code review datasets. Section~\ref{sec:noise_impact_on_comment_generation_models_rq2} explores the impact of these noisy comments on machine learning models, while Section~\ref{sec:noisy_impact_on_generated_comment_quality_rq3} evaluates the quality of comments generated by models trained on cleaned datasets. We discuss our findings and their implications in Section~\ref{sec:discussion}. Section~\ref{sec:related_work} contextualizes our work within the existing literature, and Section~\ref{sec:threats_to_validity} addresses potential threats to the validity of our study. Finally, Section~\ref{sec:conclusion} draws the conclusions. 



\begin{table*}[h]
\small 
\centering
\caption{Model Performance on Comment Generation Models.}
\label{table:comment_gen_main_results}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l|lcc|ccc|ccc}
\toprule 
\textbf{Model} & \textbf{Data Set} & \textbf{\#Training } & \textbf{\#Valid} &  \multicolumn{3}{c}{\textbf{BLEU-4}}  & \multicolumn{3}{c}{\textbf{BLEU-4 (W/O Stop) }}\\ 
~& ~ & ~ & ~ & \textbf{Test$\uparrow$} & \textbf{Valid$\uparrow$} & \textbf{Noisy$\downarrow$} & \textbf{Test$\uparrow$} & \textbf{Valid$\uparrow$} & \textbf{Noisy$\downarrow$} \\ \midrule
Transformer-b & \multirow{8}{*}{Origin} & \multirow{8}{*}{117739} & \multirow{8}{*}{10319} & 4.76 & - & - & - & - & - \\ 
Tufano et al. &  &  &  & 4.39 & - & - & - & - & - \\ 
CodeT5 &  &  &  & 4.83 & - & - & - & - & - \\ 
CommentFinder &  &  &  & 3.82 & - & - & - & - & - \\ 
CodeReviewer (Reported) &  &  &  & 5.32 & - & - & - & - & - \\ 
LLaMA-Reviewer-Prefix  &  &  &  & 5.16 & - & - & - & - & - \\ 
LLaMA-Reviewer-LoRA  &  &  &  & 5.70 & - & - & - & - & - \\ 
CCT5 (Lin et al., 2023) &  &  &  & \textbf{6.30} & - & - & - & - & - \\ \midrule 
\multirow{5}{*}{CodeReviewer} & Origin & 117739 & 10319 & 5.73 & 7.12 & 5.60 & 7.33 & 9.55 & 7.75 \\ 
 & Clean\_Llama3 & 87872 & 7571 & 5.97 & \underline{7.71} & 5.14 & \textbf{7.44} & \textbf{10.25} & 6.52 \\ 
 & Control\_Llama3 & - & - & 5.63 & 7.45 & 5.86 & 7.22 & 9.67 & 7.34 \\ 
 & Clean\_GPT-3.5 & 39625 & 3395 & \underline{6.04} & \textbf{7.99} & 4.83 & \underline{7.41} & \underline{10.07} & 5.98 \\ 
 & Control\_GPT-3.5 & - & - & 5.63 & 7.39 & 5.70 & 7.26 & 9.54 & 8.21 \\ \midrule 
\multirow{5}{*}{CodeT5} & Origin & 117739 & 10319 & 5.19 & 5.85 & 6.03 & 6.64 & 6.83 & 7.79 \\ 
 & Clean\_Llama3 & 87872 & 7571 & 5.54 & 6.09 & 5.46 & 6.87 & 7.76 & 6.79 \\ 
 & Control\_Llama3 & - & - & 5.21 & 5.38 & 5.01 & 6.45 & 6.70 & 6.06 \\ 
 & Clean\_GPT-3.5 & 39625 & 3395 & 5.67 & 6.06 & 5.15 & 6.79 & 7.41 & 5.54 \\ 
 & Control\_GPT-3.5 & - & - & 5.20 & 5.45 & 5.41 & 6.45 & 7.03 & 6.29 \\ \bottomrule 
\end{tabular}%
% }
\end{table*}







% \begin{table*}[h]
% \small 
% \centering
% \caption{Model Performance on Comment Generation Models.}
% \label{table:comment_gen_main_results}
% \setlength{\tabcolsep}{0.8pt}  % Adjust the spacing between columns here
% \resizebox{0.98\textwidth}{!}{
% \begin{tabular}{ll|lllllll|lllllll}
% \toprule 
% \textbf{$M$} & \textbf{Dataset} &  \multicolumn{7}{c|}{\textbf{BLEU-4}} & \multicolumn{7}{c}{\textbf{BLEU-4 (W/O Stop)}} \\ 
% ~ & ~ & \textbf{Test} & \textbf{Valid} & \textbf{Noisy} & \textbf{Valid$_{\text{T}}$} & \textbf{Noisy$_{\text{T}}$} & \textbf{Valid$_{\text{C}}$} & \textbf{Noisy$_{\text{C}}$} & \textbf{Test} & \textbf{Valid} & \textbf{Noisy} & \textbf{Valid$_{\text{T}}$} & \textbf{Noisy$_{\text{T}}$} & \textbf{Valid$_{\text{C}}$} & \textbf{Noisy$_{\text{C}}$} \\ \midrule
% \multirow{5}{*}{\rotatebox{90}{CodeReviewer}} & Origin & 5.73 & 5.45 & 5.17 & 7.12 & 5.60 & 6.17 & 5.41 & 7.33 & 6.80 & 6.32 & 9.55 & 7.75 & 8.04 & 6.96 \\
% ~ & Clean\_Llama3 & \underline{5.97} \ 4.2\%↑ & 5.64 \ 3.5\%↑& 5.11 \ 1.2\%↓ & \underline{7.71} \ 8.3\%↑ & 5.14  \ 8.2\%↓ & \underline{6.63} \ 7.5\%↑ & 5.18 \ 4.3\%↓ & \textbf{7.44} \ 1.5\%↑ & 7.02 \ 3.2\%↑ & 6.49 \ 2.7\%↑ & \textbf{10.25} \ 7.3\%↑ & 6.52 \ 15.9\%↓ & \underline{8.57} \ 6.6\%↑ & 6.56 \ 5.7\%↓ \\
% ~ & Control\_Llama3 & 5.63 & 5.12 & 5.36 & 7.45 & 5.86 & 6.18 & 5.66 & 7.22 & 6.48 & 6.77 & 9.67 & 7.34 & 7.95 & 7.06 \\
% ~ & Clean\_GPT-3.5&  \textbf{6.04} \ 5.4\%↑ & \textbf{5.93} \ 8.8\%↑ & 5.19 \ 0.4\%↑ & \textbf{7.99} \ 12.2\%↑ & 4.83 \ 13.8\%↓ & \textbf{6.97} \ 13.0\%↑ & 5.02 \ 7.2\%↓ & \underline{7.41} \ 1.1\%↑ & \textbf{7.40} \ 8.8\%↑ & 6.17 \ 2.4\%↓ & \underline{10.07} \ 5.4\%↑ & 5.98  \ 22.8\%↓ & \textbf{8.75} \ 8.8\%↑ & 6.08 \ 12.6\%↓\\
% ~ & Control\_GPT-3.5 & 5.63 & 5.21 & 5.13 & 7.39 & 5.70 & 6.20 & 5.43 & 7.26 & 6.48 & 6.63 & 9.54 & 8.21 & 7.89 & 7.37 \\ \midrule 
% \multirow{5}{*}{\rotatebox{90}{CodeT5}} & Origin&  5.19 & 4.84 & 5.09 & 5.85 & 6.03 & 5.34 & 5.04 & 6.64 & 5.82 & 6.88 & 6.83 & 7.79 & 6.59 & 6.75 \\ 
% ~ & Clean\_Llama3& 5.54 \ 6.7\%↑ & 5.32 \ 9.9\%↑& 5.14 \ 1.0\%↑ & 6.09 \ 4.1\%↑ & 5.46 \ 9.5\%↓ & 5.74 \ 7.5\%↑ & 5.33 \ 5.8\%↑ & 6.87 \ 3.5\%↑ & 6.63 \ 13.9\%↑ & 6.10 \ 11.3\%↓ & 7.76 \ 13.6\%↑ & 6.79 \ 12.8\%↓ & 7.24 \ 9.9\%↑ & 6.52 \ 3.4\%↓\\
% ~ & Control\_Llama3& 5.21 & 4.95 & 5.26 & 5.38 & 5.01 & 5.19 & 5.12 & 6.45 & 5.66 & 6.98 & 6.70 & 6.06 & 6.20 & 6.55 \\
% ~ & Clean\_GPT-3.5 & 5.67 \ 9.2\%↑ & \underline{5.88} \ 21.5\%↑ & 5.27 \ 3.5\%↑ & 6.06 \ 3.6\%↑ & 5.15 \ 14.6\%↓ & 6.00 \ 12.4\%↑ & 5.23 \ 3.8\%↑ & 6.79 \ 2.3\%↑ & \underline{7.17} \ 23.2\%↑ & 5.92 \ 14.0\%↓ & 7.41 \ 8.5\%↑ & 5.54 \ 28.9\%↓ & 7.32 \ 11.1\%↑ & 5.76 \ 14.7\%↓ \\
% ~ & Control\_GPT-3.5 & 5.20 & 5.17 & 5.39 & 5.45 & 5.41 & 5.34 & 5.30 & 6.45 & 6.20 & 6.68 & 7.03 & 6.29 & 6.67 & 6.33 \\ \bottomrule 
% \end{tabular}
% }
% \end{table*}




% \begin{table}[!t]
% % \small 
% \setlength{\tabcolsep}{4.5pt}
% \centering
% \begin{tabular}[width=0.45\textwidth]{l|cc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Training Set}} & \multicolumn{2}{c|}{\textbf{Information }} & \multicolumn{3}{c}{\textbf{Relevance }}  \\
% % \cline{2-8}
% % \midrule
% \cmidrule(lr){2-6} %\cmidrule(lr){5-8}
% & Valid & Noisy  & Valid & Noisy  &Test (all) \\
% \midrule
% \textsc{Original} & 3.50 & 3.40 &  2.43 & 2.54  & 3.69 \\
% \textsc{Clean\_Llama3} & 4.08 & 4.10 & 2.70 & \textbf{2.74}  & 3.85 \\
% \textsc{Control\_GPT-3.5} & \textbf{4.28} & \textbf{4.26} & \textbf{2.80} & \textbf{2.74}  & \textbf{4.38} \\
% \bottomrule
% \end{tabular}
% \caption{Information and Relevance Scores for Different Training Sets on CodeReviewer model.}
% \label{table:information_relevance_scores}
% \end{table}



\begin{table*}[h]
        \small 
        \centering
        \caption{Model Performance on Comment Generation Models.}
        \label{table:comment_gen_main_results}
        \setlength{\tabcolsep}{3pt}  % Adjust the spacing between columns here
        % \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{ll|l|ll|ll|ll}
        \toprule 
        % \textbf{$M$} & \textbf{Dataset} &  \multicolumn{7}{c}{\textbf{BLEU-4}} \\ 
        \textbf{$M$} & \textbf{Dataset} & \textbf{Test} & \textbf{Valid$_{\text{our}}$} & \textbf{Noisy$_{\text{our}}$} & \textbf{Valid$_{\text{T}}$} & \textbf{Noisy$_{\text{T}}$} & \textbf{Valid$_{\text{C}}$} & \textbf{Noisy$_{\text{C}}$}  \\ \midrule
          \multicolumn{9}{c@{}}{\textbf{BLEU-4 }} \\ \midrule 
        \multirow{5}{*}{\rotatebox{90}{CodeReviewer}} & \textsc{Origin} & 5.73 & 5.45 & 5.17 & 7.12 & 5.60 & 6.17 & 5.41  \\
        ~ & \textsc{Clean\_Llama3} & \underline{5.97} \ 4.2\%↑ & 5.64 \ 3.5\%↑& 5.11 \ 1.2\%↓ & \underline{7.71} \ 8.3\%↑ & 5.14  \ 8.2\%↓ & \underline{6.63} \ 7.5\%↑ & 5.18 \ 4.3\%↓ \\
        ~ & \textsc{Control\_Llama3} & 5.63 & 5.12 & 5.36 & 7.45 & 5.86 & 6.18 & 5.66\\
        ~ & \textsc{Clean\_GPT-3.5} &  \textbf{6.04} \ 5.4\%↑ & \textbf{5.93} \ 8.8\%↑ & 5.19 \ 0.4\%↑ & \textbf{7.99} \ 12.2\%↑ & 4.83 \ 13.8\%↓ & \textbf{6.97} \ 13.0\%↑ & 5.02 \ 7.2\%↓ \\
        ~ & Control\_GPT-3.5 & 5.63 & 5.21 & 5.13 & 7.39 & 5.70 & 6.20 & 5.43 \\ \midrule 
        \multirow{5}{*}{\rotatebox{90}{CodeT5}} & \textsc{Origin}&  5.19 & 4.84 & 5.09 & 5.85 & 6.03 & 5.34 & 5.04  \\ 
        ~ & \textsc{Clean\_Llama3}& 5.54 \ 6.7\%↑ & 5.32 \ 9.9\%↑& 5.14 \ 1.0\%↑ & 6.09 \ 4.1\%↑ & 5.46 \ 9.5\%↓ & 5.74 \ 7.5\%↑ & 5.33 \ 5.8\%↑ \\
        ~ & \textsc{Control\_Llama3}& 5.21 & 4.95 & 5.26 & 5.38 & 5.01 & 5.19 & 5.12 \\
        ~ & \textsc{Clean\_GPT-3.5} & 5.67 \ 9.2\%↑ & \underline{5.88} \ 21.5\%↑ & 5.27 \ 3.5\%↑ & 6.06 \ 3.6\%↑ & 5.15 \ 14.6\%↓ & 6.00 \ 12.4\%↑ & 5.23 \ 3.8\%↑ \\
        ~ & \textsc{Control\_GPT-3.5} & 5.20 & 5.17 & 5.39 & 5.45 & 5.41 & 5.34 & 5.30  \\  \midrule \midrule
           \multicolumn{9}{c@{}}{\textbf{BLEU-4 (W/O Stop Words)}}  \\ 
         \cmidrule(lr){1-9}  % This line adds the horizontal rule
        \multirow{5}{*}{\rotatebox{90}{CodeReviewer}} & \textsc{Origin} & 7.33 & 6.80 & 6.32 & 9.55 & 7.75 & 8.04 & 6.96 \\
        ~ & \textsc{Clean\_Llama3}  & \textbf{7.44} \ 1.5\%↑ & 7.02 \ 3.2\%↑ & 6.49 \ 2.7\%↑ & \textbf{10.25} \ 7.3\%↑ & 6.52 \ 15.9\%↓ & \underline{8.57} \ 6.6\%↑ & 6.56 \ 5.7\%↓ \\
        ~ & \textsc{Control\_Llama3} & 7.22 & 6.48 & 6.77 & 9.67 & 7.34 & 7.95 & 7.06 \\
        ~ & \textsc{Clean\_GPT-3.5} &  \underline{7.41} \ 1.1\%↑ & \textbf{7.40} \ 8.8\%↑ & 6.17 \ 2.4\%↓ & \underline{10.07} \ 5.4\%↑ & 5.98  \ 22.8\%↓ & \textbf{8.75} \ 8.8\%↑ & 6.08 \ 12.6\%↓\\
        ~ & Control\_GPT-3.5 &  7.26 & 6.48 & 6.63 & 9.54 & 8.21 & 7.89 & 7.37 \\ \midrule 
        \multirow{5}{*}{\rotatebox{90}{CodeT5}} &  \textsc{ORIGIN} &  6.64 & 5.82 & 6.88 & 6.83 & 7.79 & 6.59 & 6.75 \\ 
        ~ & \textsc{Clean\_Llama3}& 6.87 \ 3.5\%↑ & 6.63 \ 13.9\%↑ & 6.10 \ 11.3\%↓ & 7.76 \ 13.6\%↑ & 6.79 \ 12.8\%↓ & 7.24 \ 9.9\%↑ & 6.52 \ 3.4\%↓\\
        ~ & \textsc{Control\_Llama3}&  6.45 & 5.66 & 6.98 & 6.70 & 6.06 & 6.20 & 6.55 \\
        ~ & \textsc{Clean\_GPT-3.5} & 6.79 \ 2.3\%↑ & \underline{7.17} \ 23.2\%↑ & 5.92 \ 14.0\%↓ & 7.41 \ 8.5\%↑ & 5.54 \ 28.9\%↓ & 7.32 \ 11.1\%↑ & 5.76 \ 14.7\%↓ \\
        ~ & \textsc{Control\_GPT-3.5} &  6.45 & 6.20 & 6.68 & 7.03 & 6.29 & 6.67 & 6.33 \\ \bottomrule 
        \end{tabular}
        % }
        \end{table*}

==> tables/prompts.tex <==

\begin{table*}[!t]
    \centering
    \small 
    \caption{Prompt templates for noisy classification task.}
    \label{tab:prompt_templates}
    \begin{tabular}{p{\textwidth}} %p{10cm}
        \textbf{Prompt} $\|$ \textbf{Template} \\
        \toprule
         \textbf{$P_{\textsc{Definition}}$} $\|$ Your task, as an experienced code reviewer skilled in Java, Python, and C++, is to evaluate review comments generated by other developers on code changes (source or code diffs) submitted in the code review process. Your objective is to discern between ``noisy'' comments and those that are ``valid''. \\ewline 
        Valid comments are those that request code changes aimed at improving the source code. A comment is considered ``valid'' if given the input information (i.e., code diff for the code-to-comment task), it is possible for a human to understand the rationale for the related output. This means that a human evaluator is able to understand what the reviewer's comment refers to (i.e., what the problem in the submitted code diff spotted by the reviewer is). Furthermore, when an instance is valid, the comment usually specifies the types of changes, including: \\ewline 
        - Changes are needed to refactor the code to improve its quality; \\ewline 
        - Changes are needed since tests for this code must be written; \\ewline 
        - Changes are needed to better align this code to good object-oriented design principles; \\ewline 
        - Changes are needed to fix one or more bugs; \\ewline 
        - Changes are needed to improve the logging of its execution; \\ewline 
        - Changes are needed for other reasons not listed above. \\ewline 
        A comment is considered ``noisy'' if it is impossible even for a human to understand the reviewer's comment. This includes the following types of noisy comments: \\ewline 
        - Unclear comment: what the reviewer's comment is actually asking the developer is unclear. This could be because the comments are vague or irrelevant to code improvement. \\ewline 
        - No change asked: the reviewer’s comment does not request any change; \\ewline 
        - Noisy for other reasons not listed above. \\ewline
        Your evaluation should be guided by the following criteria: \\ewline 
        1. \textbf{Relevance to Code Change:} A valid comment should directly relate to the code diff submitted, specifically recommending precise alterations or improvements. You should classify the comment's suggested changes into the types listed above when a comment is identified as valid. Similarly, you should classify the discarded reason into types listed above when a comment is identified as discard. \\ewline 
        2. \textbf{Clarity and Constructiveness:} The comment should clearly articulate any identified issues and offer constructive suggestions for how to address them. \\ewline 
        3. \textbf{Focus on Improvement:} Comments should aim to enhance the code's quality by identifying defects, analyzing their potential impact, and suggesting actionable steps for remediation. \\ewline \\ewline
        This exercise involves a single-round code review process, where your primary goal is to improve the quality of feedback within the review ecosystem by filtering out noisy comments, thereby ensuring that only useful, clear, and constructive feedback is provided to developers for code enhancement. \\ 
        \midrule
        \textbf{$P_{\textsc{Guideline}}$ $\|$} As an experienced code reviewer skilled in multiple programming languages, your role during the code review process is to assess code review comments made by reviewers on code diffs, which are the code changes developers make. Review comments often highlight issues, suggest changes, and sometimes explain the reasoning behind suggested changes. Your primary objective is to determine whether each comment is ``valid'' or ``noisy''. \\ewline \\ewline
        A ``valid'' comment often explicitly requests changes to improve the code, clearly outlining necessary actions, such as refactoring the code to improve code quality (regarding documentation, style, programming conventions and more), writing tests, aligning with good object-oriented design principles, fixing bugs, enhancing logging, or addressing other specific needs. It should be straightforward to discern these actions from the comment, which often involves assessing whether the comment raises an issue or concern relevant to the code diff and identifying the specific actions being asked to improve the code. \\ewline \\ewline
        A comment is considered ``noisy'' if it fails to relate to the code diff, lacks direct and explicit requests for code improvement, or is unclear and nearly impossible to understand. These issues can arise from the comment's irrelevance, requests for mere clarifications, justifications of existing code diff, or other obstructive factors. \\ewline \\ewline
        Human experts classify comments as valid or noisy using the above high-level definition along with detailed guidelines to identify concrete aspects presented in comments and assess whether the comment is valid or noisy. Each aspect represents a potential component of a comment and includes a type name, definition, criteria for being valid, and criteria for being noisy. \\ 
        \\\\---\\ Type: Action Explicitness\\**Definition:** A criterion used to determine the explicitness of a comment regarding the need for a code change. You can extract the key verbs in comments to help you understand whether it is explicit or implicit.\\- **Valid:** A comment is considered valid if the action specified in the comment is direct and explicit, requesting a specific code change. Such comments provide clear suggestions or solutions on what to act on, leaving little room for interpretation. \\- **Noisy:** A comment is considered noisy if the action specified in the comment is indirect or implicit. These comments require further inference or speculation to discern the specific action being requested, leading to difficulty of mapping key information in comments back to code diff and a higher likelihood of misinterpretation.\\\\ Type: Questions in Comments\\**Definition:** This is a common type that frequently occurs in code review comments, where the comment is expressed as a question. Such comments might provide direct suggestions that prompt developers to take action or purely aim to seek information.\\- **Valid:**A comment is valid if it provides concrete suggestions or solutions on how to improve the relevant code. A considerable amount of questions are used to elicit an action from the developer who submitted the code diff. For example, many questions actually suggest alternative solutions. The use of a question rather than an affirmative sentence to recommend a different implementation strategy might indicate the reviewer’s attempt to be polite towards the change author. In some other cases, reviewers directly ask the change authors to perform a specific action using questions.\\- **Noisy:**  A comment expressed as a question is noisy if it doesn't lead to an action for code change or if the action is implicit, as explained below: (a) comments that request further details or clarification without directly prompting a specific course of action; (b) when the action is not explicitly stated and lacks clarity in what is being asked, requiring significant inference or speculation to deduce potential actions, which may vary widely. Evaluate this carefully as not all questions are noisy.\\\\ Type: Issue Scope\\**Definition:** This assesses the relevance regarding the scope of issue pointed out by a reviewer's comment.\\- **Valid:** A comment is valid if the issue scope is relevant to the code diff (code diff) and the action for refining the code is explicit and direct. \\- **Noisy:** A comment is noisy if the issues pointed out in the scope are irrelevant to the actual code changes, or do not provide actionable suggestions. \\\\ Type: Action Scope\\**Definition:** This defines the action or change scope asked in the comment.\\- **Valid:**  A comment is considered valid if the raised issue is relevant to the code diff, and the action being requested is direct and explicit, even if the action scope goes beyond the code diff scope.\\- **Noisy:** A comment is considered noisy if it raises issues outside the scope of the relevant code diff or if the action being requested is indirect and implicit.\\\\ Type: Programming or Package Knowledge  \\**Definition:** This type arises when the reviewer's comment requires programming language specific knowledge or package specific knowledge to understand and implement the requested changes.\\- **Valid:** A comment is valid if it provides direct, actionable suggestions and if the keywords in the comment are relevant to the code diff, file, or specific programming languages used in the code.\\- **Noisy:** A comment is noisy if no associations or connections to the domain-specific knowledge are made clear, making the feedback confusing and hard to act upon.\\\\ Type: Contributors Comments\\- **Definition:** This is a type of comment provided by contributors themselves, where they serve as reviewers.\\- **Valid:** A comment is valid if the change being requested is relevant to the code diff and is direct and explicit to apply, regardless of the source of the rationale or the existence of the rationale.\\- **Noisy:** A comment is noisy if it is a self-justification, i.e., purely clarifying what has already been done in the code and why it was done. You need to read the code and comment carefully, mapping the actions being requested in the comment to the changed lines in the code diff to understand whether it is a self-justification.\\\\ Type: Rationale Source\\- **Definition:** This is often part of a comment where the reasoning or rationale to support the suggestion comes from a scope beyond the code diff. This could be at a file level, from higher software development life cycles, or based on the reviewer's experience or conventions in a specific project or language.\\- **Valid:** A comment is valid if the change being requested is relevant to the code diff and is direct and explicit to apply, regardless of the source of the rationale or the existence of the rationale.\\- **Noisy:** A comment is noisy if it is not relevant to the code diff or if it asks for an implicit and unactionable code change.\\
        

        
        \bottomrule 
    \end{tabular}
    
\end{table*}


